PlaNet of the Bayesians: Reconsidering and Improving Deep Planning Network by Incorporating Bayesian Inference

In the present paper, we propose an extension of the Deep Planning Network (PlaNet), also referred to as PlaNet of the Bayesians (PlaNet-Bayes). There has been a growing demand in model predictive control (MPC) in partially observable environments in which complete information is unavailable because of, for example, lack of expensive sensors. PlaNet is a promising solution to realize such latent MPC, as it is used to train state-space models via model-based reinforcement learning (MBRL) and to conduct planning in the latent space. However, recent state-of-the-art strategies mentioned in MBRR literature, such as involving uncertainty into training and planning, have not been considered, significantly suppressing the training performance. The proposed extension is to make PlaNet uncertainty-aware on the basis of Bayesian inference, in which both model and action uncertainty are incorporated. Uncertainty in latent models is represented using a neural network ensemble to approximately infer model posteriors. The ensemble of optimal action candidates is also employed to capture multimodal uncertainty in the optimality. The concept of the action ensemble relies on a general variational inference MPC (VI-MPC) framework and its instance, probabilistic action ensemble with trajectory sampling (PaETS). In this paper, we extend VI-MPC and PaETS, which have been originally introduced in previous literature, to address partially observable cases. We experimentally compare the performances on continuous control tasks, and conclude that our method can consistently improve the asymptotic performance compared with PlaNet.

==> IROS2020 - Bayesian Deep Planning Network/alg.tex <==
\begin{algorithm}[h]
\footnotesize
% \small
\DontPrintSemicolon
  % \KwInput{Initial state $\state_{1}$}
  % \KwData{initial variance ~$\actions_{init}$}
  Initialize $\mathcal{D}$ with a random controller for several trials \;
  \tcp*[l]{Training loop}
  \Repeat{the MPC-policy performs well}{
  Train $\{\theta_{i}\}^{E}_{i=1}$ by optimizing Eq.~\ref{eqn:vae_elbo} \; %\tcp*[l]{latent state-space model ensemble}
  % Infer $\modelpost$ \tcp*[l]{train latent state-space model}
  Initialize $\{(\latenth_{i,0}, \latents_{i,0})\}^{E}_{i=1}$ and $\action_{0}$\ as $\mathbf{0}$s \;
  Reset environment and observe $\obs_{1}$ \;
  \tcp*[l]{Control loop, $H$: episode length}
  \For{$t \leftarrow 1$ \KwTo $H$}{
  Initialize GMM parameter $\phi^{(0)}$ \;
  Execute Alg.~\ref{alg:bplanet_inner} \;%$(\obs_{t},
  % $\phi^{(U)} \leftarrow $Exec.~Alg.~\ref{alg:bplanet_inner} \;%$(\obs_{t}, \phi^{(0)}, \modelpost)$\;
  Sample $\action_{t:t+T-1} \sim q(\action_{t:t+T-1}; \phi^{(U)})$ \;
  Send $\action_{t}$ to actuators and observe $(\obs_{t+1}, r_{t+1})$\;
  $\mathcal{D} \leftarrow \mathcal{D} \cup \{(\obs_{t}, \action_{t}, r_{t+1})\}$ \;
  }}
\caption{PlaNet-Bayes' training and control loop} \label{alg:bplanet_outer}
\end{algorithm}
%
\begin{algorithm}[h]
\footnotesize
% \small
\DontPrintSemicolon
  \KwInput{Current observation $\obs_{t}$, \\
  Previous latent states and action $\{(\latenth_{i, t-1}, \latents_{i, t-1})\}^{E}_{i=1}$, $\action_{t-1}$, \\
  Initial parameters of variational distribution~$\phi^{(0)}$}
  \KwOutput{Optimized parameters of variational distribution~$\phi^{(U)}$ \\
  Current latent states $\{(\latenth_{i, t}, \latents_{i, t})\}^{E}_{i=1}$}
  \tcp*[l]{(0) Estimate the current latent state}
  \If{$t > 1$}{
  Evolve the latent state $\{\latenth_{i,t} = f^{\mathrm{GRU}}(\latenth_{i,t-1}, \latents_{i,t-1}, \action_{t-1}; \theta_{i})\}^{E}_{i=1}$ \;
  }
  Infer the latent state $\{\latents_{i,t} \sim q(\latents_{t} | \latenth_{i,t}, \obs_{t}, \theta_{i})\}^{E}_{i=1}$ \;
  % Evolve latent $\latenth_{t} = f^{\mathrm{GRU}}(\latenth_{t-1}, \latents_{t-1}, \action_{t-1})$ \;
  % Infer latent $\latents_{t} \sim q(\latents_{t} | \latenth_{t}, \obs_{t})$ \;
  \For{$j \leftarrow 1$ \KwTo $U$}{
%   Sample actions $\{\action_{k} \sim q(\action; \phi^{(j)})\}_{k=1}^{K}$ \;
%   Sample trajectories $\{\traj_{k, i} \sim p(\state; \action, \theta)\modelpost \}_{k=1}^{K}$ \;
  \tcp*[l]{(1) Sample $K$ candidates}
  Sample actions $\{\action_{k} \sim q(\action; \phi^{(j-1)}\}_{k=1}^{K}$ \;
  \tcp*[l]{(2) Eval.~the objective for each candidate}
  Sample trajectories and rewards $\{ \{ \{$ \;
  \Indp $\latenth_{k, i, t'+1} = f_{\theta_{i}}^{\mathrm{GRU}}(\latenth_{k,i,t'}, \latents_{k,i,t'}, \action_{k,t'})$, \;
  $\latents_{k,i,t'+1} \sim p(\latents_{k,t'+1} | \latenth_{k, i, t'+1}, \theta_{i})$ \;
  $r_{k,i,t'+1} \sim p(r_{t'+1} | \latenth_{k, i, t'+1}, \latents_{k, i, t'+1})$ \;
  \Indm $\}_{t'=t}^{t+T-1} \}_{i=1}^{E}\}_{k=1}^{K}$ \;
  Calc.~trajectory rewards $\{R_{k} = \frac{1}{E}\sum^{E}_{i=1}\sum^{t+T}_{t'=t+1}r_{k,i,t'}\}^{K}_{k=1}$\;
  % Update $\actionm$ and $\actions$ by applying CEM
  \tcp*[l]{(3) Update proposal distribution}
  % Calc.~weights $\{w_{k} = \mathbbm{1}[R_{k} \geq R_{\mathrm{thd}}] \}^{K}_{k=1}$ \;
  Update $\phi^{(j)}$ by Eq.~\ref{eqn:paets}.
  % Update $\actionm \leftarrow \sum^{K}_{k=1}w_{k}\cdot\action_{k}/\sum^{K}_{k=1}w_{k}$ \;
  % Update $\actions^{2} \leftarrow \sum^{K}_{k=1}w_{k}\cdot(\action_{k}-\actionm)^{2}/\sum^{K}_{k=1}w_{k}$\;
  }
\caption{PlaNet-Bayes' latent planning with PaETS} \label{alg:bplanet_inner}
\end{algorithm}


==> IROS2020 - Bayesian Deep Planning Network/alg0.tex <==
\SetAlCapNameFnt{\footnotesize}
\SetAlCapFnt{\footnotesize}
% \SetAlCapNameFnt{\small}
% \SetAlCapFnt{\small}

\begin{algorithm}[h]
\footnotesize
% \small
\DontPrintSemicolon
  \KwInput{Current observation $\obs_{t}$, \\
  Previous latent states and action $(\latenth_{t-1}, \latents_{t-1}, \action_{t-1})$, \\
  Initial parameters of the proposal distribution~$(\actionm^{(0)}, \actions^{(0)})$}
  \KwOutput{Optimized parameters of proposal dist.~$(\actionm^{(U)}, \actions^{(U)})$ \\
  Current latent states $(\latenth_{t}, \latents_{t})$}
  \tcp*[l]{(0) Estimate current latent state}
  \If{$t > 1$}{
  Evolve the latent state $\latenth_{t} = f^{\mathrm{GRU}}(\latenth_{t-1}, \latents_{t-1}, \action_{t-1})$ \;
  }
  Infer the latent state $\latents_{t} \sim q(\latents_{t} | \latenth_{t}, \obs_{t})$ \;
  % Evolve latent $\latenth_{t} = f^{\mathrm{GRU}}(\latenth_{t-1}, \latents_{t-1}, \action_{t-1})$ \;
  % Infer latent $\latents_{t} \sim q(\latents_{t} | \latenth_{t}, \obs_{t})$ \;
  \For{$j \leftarrow 1$ \KwTo $U$}{
%   Sample actions $\{\action_{k} \sim q(\action; \phi^{(j)})\}_{k=1}^{K}$ \;
%   Sample trajectories $\{\traj_{k, i} \sim p(\state; \action, \theta)\modelpost \}_{k=1}^{K}$ \;
  \tcp*[l]{(1) Sample $K$ candidates}
  Sample actions $\{\action_{k} \sim q(\action; \actionm^{(j-1)}, \actions^{(j-1)}\}_{k=1}^{K}$ \;
  \tcp*[l]{(2) Eval.~the objective for each candidate}
  Sample trajectories and rewards $\{ \{$ \;
  \Indp $\latenth_{k, t'+1} = f^{\mathrm{GRU}}(\latenth_{t'}, \latents_{t'}, \action_{k,t'})$, \;
  $\latents_{k,t'+1} \sim p(\latents_{t'+1} | \latenth_{k, t'+1})$ \;
  $r_{k,t'+1} \sim p(r_{t'+1} | \latenth_{k, t'+1}, \latents_{k, t'+1})$ \;
  \Indm $\}_{t'=t}^{t+T-1} \}_{k=1}^{K}$ \;
  Calc.~trajectory rewards $\{R_{k} = \sum^{t+T}_{t'=t+1}r_{k,t'}\}^{K}_{k=1}$\;
  % Update $\actionm$ and $\actions$ by applying CEM
  \tcp*[l]{(3) Update proposal distribution}
  Calc.~weights $\{w_{k} = \mathds{1}[R_{k} \geq R_{\mathrm{thd}}] \}^{K}_{k=1}$ \;
  Normalize weights $\{w_{k} \leftarrow w_{k} / \sum^{K}_{k'=1}w_{k'}\}^{K}_{k=1}$ \;
  Update $(\actionm^{(j)}, (\actions^{(j)})^{2}) \leftarrow (\sum^{K}_{k=1}w_{k}\cdot\action_{k}, \sum^{K}_{k=1}w_{k}\cdot(\action_{k}-\actionm^{(j)})^{2})$ \;
  % Update $\actionm \leftarrow \sum^{K}_{k=1}w_{k}\cdot\action_{k}/\sum^{K}_{k=1}w_{k}$ \;
  % Update $\actions^{2} \leftarrow \sum^{K}_{k=1}w_{k}\cdot(\action_{k}-\actionm)^{2}/\sum^{K}_{k=1}w_{k}$\;
  }
\caption{PlaNet's latent planning based on CEM \cite{hafner2018learning}} \label{alg:planet_cem}
\end{algorithm}

